AExGym: Benchmarks and Environments for Adaptive Experimentation

Innovations across science and industry are evaluated using randomized trials (a.k.a. A/B tests). While simple and robust, such static designs are inefficient or infeasible for testing many hypotheses. Adaptive designs can greatly improve statistical power in theory, but they have seen limited adoption due to their fragility in practice. We present a benchmark for adaptive experimentation based on real-world datasets, highlighting prominent practical challenges to operationalizing adaptivity: non-stationarity, batched/delayed feedback, multiple outcomes and objectives, and external validity. Our benchmark aims to spur methodological development that puts practical performance (e.g., robustness) as a central concern, rather than mathematical guarantees on contrived instances. We release an open source library, AExGym, which is designed with modularity and extensibility in mind to allow experimentation practitioners to develop custom environments and algorithms.

==> code-package.tex <==
\section{AExGym}

In order to benchmark existing algorithms in practical settings and facilitate methodological development, we create AExGym, a software package that is meant to be accessible and flexible. AExGym is designed with the purpose of allowing experimenters to easily evaluate and develop algorithms in a customized setting. For the purpose of evaluation, we first provide an environment interface that can easily incorporate existing data, customized objectives and constraints. To facilitate the implementation and development of algorithms, ... 

\subsection{Environment}
Adaptive experiments involve a sequential decision making process where at each step, an experimenter makes a decision based on existing information, and receives some form of tangible feedback from an environment. To enable the simulation of such a process, we create a "Gym" environment modeled after the OpenAI Gym \cite{BrockmanChPeScScTaZa16}, tailored for adaptive experimentation problems.

While the OpenAI Gym involves a general observation $O_{t}$ at each decision making stage $t$, we add more structure to our environment by giving the option to provide contexts $x_{i}$ corresponding to the batch of ${n_{t}}$ sampling units to be assigned a treatment arm, action features $z_{a}$ corresponding to potential actions, costs $c_{x, a}$ associated with taking action $a$ on unit $x$, and distributions of future contexts $\mu_{t+1:T}$. We emphasize that each component can be omitted based on an experimenter's needs, but we offer functionality for each as they are widely used in experiment decisions. After treatment allocation decisions have been made, the environment provides rewards $\{R(x_{i}, a_{i})\}_{i=1}^{n_{t}}$.  

\begin{example}
    To elucidate upon these design choices, consider the Pennsylvania Reemployment Bonus Demonstration \cite{corson1991pennsylvania}, an experiment testing the efficacy of various reemployment bonuses on unemployed individuals. At each decision making stage, one may have access to (1) personal information $x_{i}$ of $n_{t}$ individuals that must be assigned a treatment group, (2) action features $z_{a}$ corresponding to the reemployment bonus amount, (3) costs $c_{x,a}$ associated with giving individual $x$ a bonus $a$, and (4) distributions of future individuals $\mu_{t+1:T}$. Knowledge of future distributions could include information about future sites of experimentation (e.g. counties, schools, etc. ). Finally, the rewards $\{R(x_{i}, a_{i})\}_{i=1}^{n_{t}}$ can include the time spent on Unemployment Insurance (UI), employment, and future earnings. 
\end{example}

\subsection{Algorithm Design}
True environment dynamics are complex and experiments universally lack the data to learn these dynamics. Therefore, adaptive experimentation algorithms maintain simpler models of the environment in order to make tractable decisions. At each decision making stage $t$, common adaptive experimentation algorithms make decisions based on feature maps $\phi(x,a)$ and a belief about interactions between the optimal parameter $\theta^{*}$ in \eqref{eq:reward-model} of some assumed parametric model. Consider the following examples of popular posterior sampling and UCB algorithms. 

\begin{example}
    (Linear Thompson Sampling) Given a belief $N(\theta_{t}, \Sigma_{t})$ at stage $t$, Linear TS chooses an action by sampling $\hat{\theta}_{t} \sim N(\theta_{t}, \Sigma_{t})$ and playing $\argmax_{a} \{\phi(x,a)^\top \hat{\theta}_{t} \}$. 
\end{example}

\begin{example}
    (Linear UCB) Given coefficient and covariance beliefs $(\theta_{t}, \Sigma_{t})$, Linear UCB chooses an action as $\argmax_{a} \{\phi(x,a)^\top \hat{\theta}_{t} + \alpha \sqrt{\phi(x,a)^\top \Sigma_{t} \phi(x,a)} \}$ where $\alpha > 0$. 
\end{example}

A key feature of these methods is that they provide an allocation policy given any belief state and feature map. To maximize modularity and flexibility, we differentiate between two modules in $\mathsf{AExGym}$:  $\mathsf{policy}$ and $\mathsf{mdp}$. Methods implemented within the $\mathsf{policy}$ module take a belief state and a feature map, and output potential actions. $\mathsf{mdp}$ classes provide the underlying feature map $\phi(\cdot)$ and determine how belief states update throughout the experiment. 

$\mathsf{mdp}$ and $\mathsf{policy}$ classes that rely on the same model (e.g. linear, logistic, etc.) should always be compatible with each other. Given a method like Linear TS, an experimenter can easily test its performance under multiple ways of linearly modeling an environment, simply by passing in various instantiations of $\mathsf{mdp}$. Likewise, experimenters can test multiple algorithms easily under one model. We give code examples: 







==> macros/new_bib <==
@article{WangClLiFr20,
  title={Parallel Bayesian Global Optimization of Expensive Functions},
  author={Jialei Wang and Scott C. Clark and Eric Liu and Peter I. Frazier},
  journal={Operations Research},
  volume=68,
  number=6,
  pages={1850--1865},
  year=2020
}

@inproceedings{Mockus05,
  title={On bayesian methods for seeking the extremum},
  author={Jonas Mo{\v{c}}kus},
  booktitle="Optimization Techniques IFIP Technical Conference Novosibirsk, July 1--7, 1974",
  year = 1975,
  publisher="Springer Berlin Heidelberg",
  address="Berlin, Heidelberg",
  pages="400--404"
}

@techreport{GinsbourgerRiCa08,
  author = {David Ginsbourger and Rodolphe Le Riche and Laurent Carraro},
  title = {A Multi-points Criterion for Deterministic Parallel Global Optimization based on Gaussian Processes},
  year = 2008,
  number = {HAL-00260579},
}

@inproceedings{WuFr16,
  author = {Jian Wu and Peter I. Frazier},
  title = "The Parallel Knowledge Gradient Method for Batch Bayesian Optimization",
  booktitle = nips16,
  year = 2016
}

@inproceedings{GonzalezDaHeLa16,
  author = {Javier Gonzalez and Zhenwen Dai and Philipp Hennig and Neil Lawrence},
  title = "Batch Bayesian Optimization via Local Penalization",
  booktitle = aistat16,
  year = 2016
}

@inproceedings{WuFr19,
  author = {Jian Wu and Peter I. Frazier},
  title = "Practical two-step look-ahead Bayesian optimization",
  booktitle = nips19,
  year = 2019
}

@inproceedings{GonzalezOsLa16,
  author = {Javier Gonzalez and Michael Osborne and Neil Lawrence},
  title = "GLASSES: Relieving The Myopia Of Bayesian Optimisation",
  booktitle = aistat16,
  year = 2016
}

@inproceedings{JiangChGoGa20,
  author = {Shali Jiang and Henry Chai and Javier González and Roman Garnett},
  title = "BINOCULARS for Efficient, Nonmyopic Sequential Experimental Design",
  booktitle = icml20,
  year = 2020
}

@inproceedings{LamWiWo16,
  author = {Remi R. Lam and Karen E. Willcox and David H. Wolpert},
  title = "Bayesian optimization with a finite budget: an approximate dynamic programming approach. ",
  booktitle = nips16,
  year = 2016
}

@inproceedings{YueAl20,
  author = {Xubo Yue and Raed AL Kontar},
  title = "Why Non-myopic Bayesian Optimization is Promising and How Far Should We Look-ahead? A Study via Rollout",
  booktitle = aistat20,
  year = 2020
}

@inproceedings{JiangJiBaKaGaGa19,
  author = {Shali Jiang and Daniel Jiang and Maximilian Balandat and Brian Karrer and Jacob Gardner and Roman Garnett},
  title = "Efficient Nonmyopic Bayesian Optimization via One-Shot Multi-Step Trees",
  booktitle = nips20,
  year = 2020
}




==> setting.tex <==
\section{Setting}
We consider adaptive experiment settings composed of $T$ sequential epochs. At each epoch $t = 0,\dots T-1$, a batch of $n_t$ sampling units arrive and there are $K_{t}$ possible arms to assign each unit. Each unit has a context $x_{i}\in \mathbb{R}^{p}$ drawn from a distribution $\mu_{t}$. Examples of contexts could include geographical attributes of a particular site, highly individual-specific features, or features describing temporal trends such as day of the week effects. Assigning an action $a\in [K]$ to $x_{i}$ yields a noisy reward $R(x_{i}, a_{i})$. 

Experimenters typically impose modeling assumptions to make valid decisions when data are limited. We assume that the experimenter uses the following general model: 
\begin{equation}
    \label{eq:reward-model}
    R(x_{i}, a_{i}) = g(\phi(x,a)^\top \theta^{*}) + \varepsilon_{i}, 
\end{equation}
where $\varepsilon_{i}$ is a noise term with $\text{Var}(\varepsilon_{i})=s^{2}$, $\phi(x,a)\in \R^{d}$ is a known feature map, $g$ is a link function, and $\theta^{*}\in \Theta\subseteq \mathbb{R}^d$ is an unknown linear coefficient unknown to the experimenter.

This setup is highly expressive and enables an experimenter to specify a wide range of custom models, including linear and logistic contextual bandits. To model settings where each treatment arm $a$ has a separate coefficient $\theta_{a}^{*}$, one could let $\theta^{*} = (\theta_{1}^{*}, ... \theta_{K}^{*})$ and easily engineer $\phi(\cdot)$ such that $\phi(x,a)^\top \theta^{*} = x^\top \theta_{a}$. To model treatment effects with non-stationary confounders, one could let $\theta^{*} = (\beta, \theta_{1}, ... \theta_{K})$ such that $\phi(x,a)^\top \theta^{*} = \beta^\top x + \theta_{a}$. Furthermore, $\phi(\cdot)$ could be an encoding from a neural network or a large, pre-trained model.

This modeling setup forms the foundation of widely used adaptive experimentation algorithms: 
\begin{enumerate}
    \item Posterior Sampling: Thompson Sampling (TS) \cite{Thompson33}, Linear TS \cite{agrawal13thompson}, NeuralTS
    \item Upper Confidence Bound / Successive Elimination: 
    \item Random Exploration: Random sampling, $\varepsilon$-greedy. Even though exploration decisions may not depend on context, final allocation decisions depend on the model \eqref{eq:reward-model}. 
\end{enumerate}

\subsection{Experimental Objectives}


==> supplementary_material.tex <==
\section*{Checklist}
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} Please see section~\ref{section:limitations}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}. Yes, we mention in Section~\ref{section:dataset_details}.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

% \section{Appendix}

% Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

% \begin{enumerate}

% \item Submission introducing new datasets must include the following in the supplementary materials:
% \begin{enumerate}
%   \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
%   \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
%   \item URL to Croissant metadata record documenting the dataset/benchmark available for viewing and downloading by the reviewers. You can create your Croissant metadata using e.g. the Python library available here: https://github.com/mlcommons/croissant
%   \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
%   \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
% \end{enumerate}

% \item To ensure accessibility, the supplementary materials for datasets must include the following:
% \begin{enumerate}
%   \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
%   \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
%   \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
%   \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
%   \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
%   \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
% \end{enumerate}

% \item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

% \item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
% \end{enumerate}
